Machine Translation Meta Evaluation through Translation Accuracy Challenge Sets

Recent machine translation (MT) metrics calibrate their effectiveness by correlating with human judgement but without any insights about their behaviour across different error types. Challenge sets are used to probe specific dimensions of metric behaviour but there are very few such datasets and they either focus on a limited number of phenomena or a limited number of language pairs. We introduce ACES, a contrastive challenge set spanning 146 language pairs, aimed at discovering whether metrics can identify 68 translation accuracy errors. These phenomena range from simple alterations at the word/character level to more complex errors based on discourse and real-world knowledge. We conduct a large-scale study by benchmarking ACES on 50 metrics submitted to the WMT 2022 and 2023 metrics shared tasks. We benchmark metric performance, assess their incremental performance over successive campaigns, and measure their sensitivity to a range of linguistic phenomena. We also investigate claims that Large Language Models (LLMs) are effective as MT evaluators by evaluating on ACES. Our results demonstrate that different metric families struggle with different phenomena and that LLM-based methods fail to demonstrate reliable performance. Our analyses indicate that most metrics ignore the source sentence, tend to prefer surface-level overlap and end up incorporating properties of base models which are not always beneficial. We expand ACES to include error span annotations, denoted as SPAN-ACES and we use this dataset to evaluate span-based error metrics showing these metrics also need considerable improvement. Finally, we provide a set of recommendations for building better MT metrics, including focusing on error labels instead of scores, ensembling, designing strategies to explicitly focus on the source sentence, focusing on semantic content and choosing the right base model for representations.

==> tables/analysis_language_pairs.tex <==
\begin{table}[ht]
\small
\centering
\setlength{\tabcolsep}{1.5pt}
\setlength{\fboxsep}{0.5pt} % Reduces the size of the colorbox cell shading
\begin{tabular}{@{}lcccc@{}}
\toprule
                    & \textbf{trained} & \textbf{en-x} & \textbf{x-en} & \textbf{x-y}         \\
\midrule
\textit{\textbf{Examples}}          & 8871  & 12695                   & 17966                   & 5815                    \\ \midrule
BLEU                    & \phantom{-}0.009 & \phantom{-}0.225                   & -0.370                  & -0.121                  \\
f101spBLEU              & \phantom{-}0.148  & \phantom{-}0.170                   & -0.290                  & -0.022                  \\
f200spBLEU              & \phantom{-}0.140  & \phantom{-}0.442                   & -0.286                  & -0.004                  \\
chrF                    & \phantom{-}0.325  & \phantom{-}0.392                   & -0.047                  & \phantom{-}0.098                   \\
BERTScore               & \phantom{-}0.479  & \phantom{-}0.031                   & \phantom{-}0.173                   & \phantom{-}0.125                   \\
BLEURT-20               & \phantom{-}0.541  & \phantom{-}0.327                   & \phantom{-}0.280                   & \phantom{-}0.257                   \\
COMET-20                & \phantom{-}0.495  & \phantom{-}0.379                   & \phantom{-}0.278                   & \phantom{-}0.121                   \\
COMET-QE 			    & \phantom{-}0.356  & \phantom{-}0.166                   & \phantom{-}0.144                   & \phantom{-}0.168                   \\
YiSi-1                  & \phantom{-}0.476  & \phantom{-}0.520                   & \phantom{-}0.185                   & \phantom{-}0.150                   \\ \midrule
COMET-22                & \phantom{-}0.599  & \phantom{-}0.486                   & \phantom{-}0.554                   & \phantom{-}0.355                   \\
metricx\_xl\_DA\_2019   & \phantom{-}0.622  & \phantom{-}0.458                   & \phantom{-}0.456                   & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.551}}                   \\
metricx\_xl\_MQM\_2020  & \phantom{-}0.608  & \phantom{-}0.567                   & \phantom{-}0.452                   & \phantom{-}0.509                   \\
metricx\_xxl\_DA\_2019  & \phantom{-}0.631  & \phantom{-}0.431                   & \phantom{-}0.462                   & \phantom{-}0.528                   \\
metricx\_xxl\_MQM\_2020 & \phantom{-}0.605  & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.572}}                   & \phantom{-}0.487                   & \phantom{-}0.502                   \\
MS-COMET-22             & \phantom{-}0.415  & \phantom{-}0.312                   & \phantom{-}0.323                   & \phantom{-}0.117                   \\
UniTE                   & \phantom{-}0.635  & \phantom{-}0.452                   & \phantom{-}0.406                   & \phantom{-}0.283                   \\
UniTE-ref               & \phantom{-}0.619  & \phantom{-}0.313                   & \phantom{-}0.413                   & \phantom{-}0.305                   \\ \midrule
COMETKiwi               & \phantom{-}0.620  & \phantom{-}0.510                   & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.694}}                   & \phantom{-}0.468                   \\
Cross-QE                & \phantom{-}0.598  & \phantom{-}0.401                   & \phantom{-}0.552                   & \phantom{-}0.291                   \\
HWTSC-Teacher-Sim       & \phantom{-}0.497  & \phantom{-}0.357                   & \phantom{-}0.352                   & \phantom{-}0.149                   \\
HWTSC-TLM               & \phantom{-}0.538  & \phantom{-}0.519                   & \phantom{-}0.167                   & \phantom{-}0.194                   \\
KG-BERTScore            & \phantom{-}0.485  & \phantom{-}0.428                   & \phantom{-}0.507                   & \phantom{-}0.347                   \\
MS-COMET-QE-22          & \phantom{-}0.483  & \phantom{-}0.488                   & \phantom{-}0.411                   & \phantom{-}0.257                   \\
UniTE-src               & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.658}}  & \phantom{-}0.445                   & \phantom{-}0.582                   & \phantom{-}0.328                   \\ \midrule
MATESE                  & -0.281 & \phantom{-}n/a                   & n/a & n/a \\
MEE                     & -0.078 & n/a & n/a & n/a \\
MEE2                    & \phantom{-}0.340  & n/a & n/a & n/a \\
MEE4                    & \phantom{-}0.391  & n/a & n/a & n/a \\
REUSE     & \phantom{-}0.430  & n/a & n/a & n/a \\
MATESE-QE & -0.313 & n/a & n/a & n/a \\ 

\bottomrule
\end{tabular}
\caption{Average Kendall’s tau-like correlation results grouped by language pairs: trained language pairs (en-de, en-ru, zh-en), from English (en-x), into English (x-en) and language pairs not involving English (x-y).  The horizontal lines delimit baseline metrics (top), all language pairs participating reference-based metrics (second), all language pairs participating reference-free metrics (third) and trained language pairs only metrics (bottom). The best result for each category is denoted by bold text with a green highlight.}
\label{tab:analysis_langpairs}
\end{table}

==> tables/analysis_mistranslation_2022.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\setlength{\fboxsep}{0.5pt} % Reduces the size of the colorbox cell shading
\begin{tabular}{@{}lccc@{}}
\toprule
                    & \hyperref[sec:discourse]{\textbf{disco.}} & \hyperref[sec:hallucination]{\textbf{halluci.}} & \textbf{other}         \\ \midrule
\textit{\textbf{Examples}}          & \textit{3698}   & \textit{10270} & \textit{10489} \\ \midrule
BLEU                    & -0.048                                         & -0.420                                             & -0.251                                     \\
f101spBLEU              & \phantom{-}0.105                                          & -0.206                                             & -0.153                                     \\
f200spBLEU              & \phantom{-}0.094                                          & -0.191                                             & -0.149                                     \\
chrF                    & \phantom{-}0.405                                          & -0.137                                             & \phantom{-}0.161                                      \\
BERTScore               & \phantom{-}0.567                                          & -0.058                                             & \phantom{-}0.362                                      \\
BLEURT-20               & \phantom{-}0.695                                          & \phantom{-}0.142                                              & \phantom{-}0.402                                      \\
COMET-20                & \phantom{-}0.641                                          & \phantom{-}0.016                                              & \phantom{-}0.399                                      \\
COMET-QE                & \phantom{-}0.666                                          & \phantom{-}0.303                                              & \phantom{-}0.208                                      \\
YiSi-1                  & \phantom{-}0.609                                          & \phantom{-}0.019                                              & \phantom{-}0.368                                      \\
\midrule
COMET-22                & \phantom{-}0.682                                          & \phantom{-}0.461                                              & \phantom{-}0.542                                      \\
metricx\_xl\_DA\_2019   & \phantom{-}0.701                                          & \phantom{-}0.493                                              & \phantom{-}0.458                                      \\
metricx\_xl\_MQM\_2020  & \phantom{-}0.573                                          & \phantom{-}0.677                                              & \phantom{-}0.394                                      \\
metricx\_xxl\_DA\_2019  & \phantom{-}0.768                                          & \phantom{-}0.541                                              & \phantom{-}0.463                                      \\
metricx\_xxl\_MQM\_2020 & \phantom{-}0.716                                          & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.713}}                                              & \phantom{-}0.392                                      \\
MS-COMET-22             & \phantom{-}0.645                                          & \phantom{-}0.148                                              & \phantom{-}0.360                                      \\
UniTE                   & \phantom{-}0.746                                          & \phantom{-}0.322                                              & \phantom{-}0.424                                      \\
UniTE-ref               & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.776}}                                          & \phantom{-}0.396                                              & \phantom{-}0.437                                      \\
\midrule
COMETKiwi               & \phantom{-}0.733                                          & \phantom{-}0.493                                              & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.637}}                                      \\
Cross-QE                & \phantom{-}0.644                                          & \phantom{-}0.395                                              & \phantom{-}0.563                                      \\
HWTSC-Teacher-Sim       & \phantom{-}0.594                                          & \phantom{-}0.296                                              & \phantom{-}0.330                                      \\
HWTSC-TLM               & \phantom{-}0.756                                          & \phantom{-}0.306                                              & \phantom{-}0.151                                      \\
KG-BERTScore            & \phantom{-}0.593                                          & \phantom{-}0.387                                              & \phantom{-}0.472                                      \\
MS-COMET-QE-22          & \phantom{-}0.626                                          & \phantom{-}0.243                                              & \phantom{-}0.416                                      \\
UniTE-src               & \phantom{-}0.772                                          & \phantom{-}0.463                                              & \phantom{-}0.551                                      \\
\midrule
Average                 & \phantom{-}0.586                                          & \phantom{-}0.242                                              & \phantom{-}0.331                                     \\
\bottomrule
\end{tabular}
\caption{2022 Results. Average Kendall’s tau-like correlation results for the sub-level categories in mistranslation: \hyperref[sec:discourse]{\textbf{disco}urse-level}, \hyperref[sec:hallucination]{\textbf{halluci}nation}, and \textbf{other} errors.  The horizontal lines delimit baseline metrics (top), participating reference-based metrics (middle) and participating reference-free metrics (bottom). The best result for each category is denoted by bold text with a green highlight. Note that \textit{Average} is an average over averages.}
\label{tab:analysis_mistranslation_2022}
\end{table}


==> tables/analysis_mistranslation_2023.tex <==
\begin{table}[h!]
\centering
\small
\setlength{\tabcolsep}{5pt}
\setlength{\fboxsep}{0.5pt} % Reduces the size of the colorbox cell shading
\begin{tabular}{@{}lccc@{}}
\toprule
                    & \hyperref[sec:discourse]{\textbf{disco.}} & \hyperref[sec:hallucination]{\textbf{halluci.}} & \textbf{other}         \\
\midrule
\textbf{\textit{Examples}}           & \textbf{\textit{3698}}                                           & \textbf{\textit{10270}}                                              & \textbf{\textit{10489}}                                      \\
\midrule
BERTscore          & \phantom{-}0.563                                          & -0.062                                             & \phantom{-}0.361                                      \\
BLEU               & -0.042                                         & -0.418                                             & -0.250                                     \\
BLEURT-20          & \phantom{-}0.695                                          & \phantom{-}0.141                                              & \phantom{-}0.398                                      \\
chrF               & \phantom{-}0.406                                          & -0.138                                             & \phantom{-}0.160                                      \\
COMET-22           & \phantom{-}0.657                                          & \phantom{-}0.113                                              & \phantom{-}0.383                                      \\
CometKiwi          & \phantom{-}0.779                                          & \phantom{-}0.465                                              & \phantom{-}0.580                                      \\
f200spBLEU         & \phantom{-}0.095                                          & -0.190                                             & -0.150                                     \\
MS-COMET-QE-22     & \phantom{-}0.631                                          & \phantom{-}0.240                                              & \phantom{-}0.417                                      \\
Random-sysname     & -0.117                                         & -0.122                                             & -0.111                                     \\
YiSi-1             & \phantom{-}0.608                                          & \phantom{-}0.017                                              & \phantom{-}0.366                                      \\
\midrule
eBLEU              & \phantom{-}0.374                                          & -0.166                                             & \phantom{-}0.282                                      \\
embed\_llama       & -0.089                                         & -0.140                                             & \phantom{-}0.189                                      \\
MetricX-23         & \phantom{-}0.757                                          & \phantom{-}0.663                                              & \phantom{-}0.393                                      \\
MetricX-23-b       & \phantom{-}0.749                                          & \phantom{-}0.656                                              & \phantom{-}0.390                                      \\
MetricX-23-c       & \phantom{-}0.694                                          & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.755}}                                              & \phantom{-}0.477                                      \\
partokengram\_F    & -0.062                                         & -0.101                                             & 0.027                                      \\
tokengram\_F       & \phantom{-}0.396                                          & -0.132                                             & \phantom{-}0.157                                      \\
XCOMET-Ensemble    & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.791}}                                          & \phantom{-}0.566                                              & \phantom{-}0.626                                      \\
XCOMET-XL          & \phantom{-}0.706                                          & \phantom{-}0.482                                              & \phantom{-}0.521                                      \\
XCOMET-XXL         & \phantom{-}0.609                                          & \phantom{-}0.540                                              & \phantom{-}0.504                                      \\
XLsim              & \phantom{-}0.217                                          & -0.066                                             & \phantom{-}0.236                                      \\
\midrule
cometoid22-wmt21   & \phantom{-}0.782                                          & \phantom{-}0.286                                              & \phantom{-}0.400                                      \\
cometoid22-wmt22   & \phantom{-}0.748                                          & \phantom{-}0.290                                              & \phantom{-}0.423                                      \\
cometoid22-wmt23   & \phantom{-}0.758                                          & \phantom{-}0.223                                              & \phantom{-}0.478                                      \\
CometKiwi-XL       & \phantom{-}0.752                                          & \phantom{-}0.501                                              & \phantom{-}0.602                                      \\
CometKiwi-XXL      & \phantom{-}0.735                                          & \phantom{-}0.535                                              & \phantom{-}0.661                                      \\
GEMBA-MQM          & \phantom{-}0.076                                          & \phantom{-}0.291                                              & \phantom{-}0.127                                      \\
KG-BERTScore       & \phantom{-}0.685                                          & \phantom{-}0.466                                              & \phantom{-}0.580                                      \\
MetricX-23-QE      & \phantom{-}0.728                                          & \phantom{-}0.604                                              & \phantom{-}0.628                                      \\
MetricX-23-QE-b    & \phantom{-}0.694                                          & \phantom{-}0.617                                              & \phantom{-}0.666                                      \\
MetricX-23-QE-c    & \phantom{-}0.747                                          & \phantom{-}0.659                                              & \colorbox[HTML]{B2EAB1}{\textbf{\phantom{-}0.739}}                                      \\
XCOMET-QE-Ensemble & \phantom{-}0.702                                          & \phantom{-}0.558                                              & \phantom{-}0.651                                      \\
XLsimQE            & \phantom{-}0.053                                          & \phantom{-}0.050                                              & \phantom{-}0.134                                      \\
\midrule
Average            & \phantom{-}0.511                                          & \phantom{-}0.248                                              & \phantom{-}0.365     \\
\bottomrule
\end{tabular}
\caption{2023 Results. Average Kendall’s tau-like correlation results for the sub-level categories in mistranslation: \textbf{disco}urse-level, \textbf{halluci}nation, and \textbf{other} errors. Metrics are grouped into baseline (top), and participating reference-based (middle) and reference-free (bottom) metrics. Note that \textit{Average} is an average over averages. Best results are highlighted in green.}
\label{tab:analysis_mistranslation_2023}
\end{table}


==> tables/zero_shot.tex <==
\begin{table}[h]
\centering
\small
%    \resizebox{\linewidth}{!}{%

\begin{tabular}{lccc}
\toprule
 &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}\hyperref[sec:antonym]{antonym-}\\ \hyperref[sec:antonym]{replacement}\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}\hyperref[subsec:real-world-commonsense]{real-world}\\ \hyperref[subsec:real-world-commonsense]{knowledge}\\ \hyperref[subsec:real-world-commonsense]{commonsense}\end{tabular}} &
  \multicolumn{1}{l}{\hyperref[sec:nonsense]{nonsense}} \\ \midrule
\textit{Examples}           & \textit{131}    & \textit{201}    & \textit{239}    \\ \midrule
BERTScore               & \phantom{-} 0.032  & -0.054 & \phantom{-} 1.469  \\
BLEURT-20               & \phantom{-} 0.032  & \phantom{-} 0.201  & \phantom{-} 0.350  \\
COMET-20                & \phantom{-} 0.048  & \phantom{-} 0.067  & \phantom{-} 1.021  \\
COMET-QE                & -0.048 & -0.188 & -0.294 \\
COMET-22                & \phantom{-} 0.080  & \phantom{-} 0.027  & \phantom{-} 0.531  \\ \midrule
metricx\_xl\_DA\_2019   & -0.032 & -0.054 & \phantom{-} 0.434  \\ 
metricx\_xl\_MQM\_2020  & -0.048 & -0.094 & \phantom{-} 0.182  \\
metricx\_xxl\_DA\_2019  & \phantom{-} 0.016  & -0.040 & \phantom{-} 0.266  \\
metricx\_xxl\_MQM\_2020 & \phantom{-} 0.064  & -0.067 & \phantom{-} 0.196  \\
UniTE-ref               & -0.032 & \phantom{-} 0.013  & \phantom{-} 0.238  \\
UniTE                   & \phantom{-} 0.080  & \phantom{-} 0.000  & \phantom{-} 0.643  \\ \midrule
COMETKiwi               & \phantom{-} 0.048  & -0.027 & \phantom{-} 0.042  \\
Cross-QE                & \phantom{-} 0.064  & \phantom{-} 0.188  & \phantom{-} 0.182  \\
HWTSC-Teacher-Sim       & \phantom{-} 0.208  & \phantom{-} 0.081  & \phantom{-} 0.350  \\
UniTE-src               & \phantom{-} 0.096  & \phantom{-} 0.161  & -0.028 \\ \bottomrule
\end{tabular}%}
\caption{Correlation difference between the performance of WMT and non-WMT language pairs reported for trained metrics across a subset of examples. $\delta$= $\tau_{\text{WMT}}$ - $\tau_{\text{non WMT}}$. WMT language pairs consist of a subset of languages seen during training of the metrics, while non-WMT language pairs are unseen. Results show that the metrics are able to generalise to unseen languages. }
\label{tab:zero-shot}
\end{table}
